HTVM: Efficient Neural Network Deployment On Heterogeneous TinyML Platforms

Optimal deployment of deep neural networks (DNNs) on state-of-the-art Systems-on-Chips (SoCs) is crucial for tiny machine learning (TinyML) at the edge. The complexity of these SoCs makes deployment non-trivial, as they typically contain multiple heterogeneous compute cores with limited, programmer-managed memory to optimize latency and energy efficiency. We propose HTVM - a compiler that merges TVM with DORY to maximize the utilization of heterogeneous accelerators and minimize data movements. HTVM allows deploying the MLPerf(TM) Tiny suite on DIANA, an SoC with a RISC-V CPU, and digital and analog compute-in-memory AI accelerators, at 120x improved performance over plain TVM deployment.

==> tables/Table_NetworksH.tex <==
\begin{table*}[t]
\label{tab:networkperformance}
\caption{Performance comparison of deployed MLPerf\textsuperscript{TM} Tiny benchmarks in different configurations. \mv{add sotA columns from ML commons?}}
\begin{tabular}{l|rr|rr|rr|rr|}
Benchmark           & \multicolumn{2}{c|}{DSCNN}            & \multicolumn{2}{c|}{MobileNet}         & \multicolumn{2}{c|}{Resnet20} & \multicolumn{2}{c|} {ToyAdmos} \\
                    & \multicolumn{2}{c|}{Keyword Spotting} & \multicolumn{2}{c|}{Visual Wake Words} & \multicolumn{2}{c|}{Image Classification} & \multicolumn{2}{c|} {Anomaly Detection} \\
                    & \multicolumn{1}{c|}{Latency} & \multicolumn{1}{c|}{Binary Size} & \multicolumn{1}{c|}{Latency} & \multicolumn{1}{c|}{Binary Size} & \multicolumn{1}{c|}{Latency} & \multicolumn{1}{c|}{Binary Size} & \multicolumn{1}{c|}{Latency} & \multicolumn{1}{c|}{Binary Size}\\
                    & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(kB)} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(kB)} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(kB)} & \multicolumn{1}{c|}{(ms)} & \multicolumn{1}{c|}{(kB)} \\
\end{tabular}
\end{table*}

==> text/Listing_DORY.tex <==
\begin{listing}[tb]
\begin{minted}[mathescape,
              linenos,
              escapeinside=||,
              highlightlines={4},
              numbersep=5pt,
              gobble=2,
              frame=lines,
              fontsize=\footnotesize,
              framesep=2mm]{python}
To do():
\end{minted}
    \caption{BYOC Dory passes of HTVM.}
    \label{listing:dory}
%\vspace{-0.4cm}
 \end{listing}
 

==> text/Listing_default_pipeline.tex <==
\begin{listing}[tb]
\begin{minted}[mathescape,
              linenos,
              escapeinside=||,
              highlightlines={4},
              numbersep=5pt,
              gobble=2,
              frame=lines,
              fontsize=\footnotesize,
              framesep=2mm]{python}
To do():
\end{minted}
    \caption{Default deployment pipeline passes of HTVM.}
    \label{listing:default}
%\vspace{-0.4cm}
 \end{listing}
 

==> text_bullets/Methods.tex <==
\section{Neural Network Compiler for Heterogeneous Computing}
Short Overview of the compilation flow.

What goes in, what comes out?

TVM $\rightarrow$ 2 paths
\begin{enumerate}
    \item Accelerator-specific codegen
    \item CPU-specific fallback codegen
\end{enumerate}

See figure \ref{fig:compilation_flow} for an overview of the compilation flow


\begin{figure}
    \centering
    \includegraphics[scale=0.4]{images/placeholder_for_comp_flow.pdf}
    \caption{Placeholder figure for the compilation flow diagram}
    \label{fig:compilation_flow}
\end{figure}

You can try out our code\footnote{Our compilation flow is open source at \texttt{url}}

\subsection{Frontend}

{\color{red}currently not automated + QAT is future work/ out of scope}

\begin{itemize}
    \item Reads in Annotated ONNX graph (ONNX no support for custom datatypes?)
    \item Graph is converted into TVM Relay IR, a DAG-IR
    \item The annotated graph is made to be matched with accelerator spec operations
\end{itemize}
\subsection{Dispatch Region detection and application}
\textit{This section is bound to change}
\begin{itemize}
    \item {\color{red}Now we do pattern matching on a predefined graph pattern $\rightarrow$ always matches. But we use as spec for testing.}
    \item Use Relay pattern matcher to find again the accelerator offloadable sections
\end{itemize}
\subsubsection{General Purpose Patterns}
\begin{itemize}
    \item Unmatched operations are codegenned with standard TVM compilation flow (Relay $\rightarrow$ TensorIR $\rightarrow$ C-code).
    \item Standard \texttt{cpu} device in TVM is optimized for X86, so we use \texttt{arm\_cpu} instead.
    \item C code is compiled with GCC (O3?) 
    \item {\color{red}Offload to PULP-NN library with BYOC?}
\end{itemize}
\subsubsection{Accelerator Specific Patterns}
\begin{itemize}
    \item Use BYOC flow 
    \item Match on operation patterns, (e.g. \texttt{conv2d + shift + clip}) + use data-types to select between different accelerators (e.g. \texttt{int2} is matched to ANIA, \texttt{int8} is matched to SOMA).
          Relay $\rightarrow$ Dory-graph $\rightarrow$ C-code 
\end{itemize}
\subsection{Edge platforms optimizations}
\begin{itemize}
    \item We use the microTVM C runtime, which was optimized for bare-metal self-contained NN deployment. (link to microTVM website?)
    \item uses optimized primitives (hardware loops and post-load increment (see PULP paper?) {\color{red} We should be careful when reporting about this, since it is not really our work}.
    \item Dory tiles the memory with linear programming (refer to Dory paper for full approach):
    Special heuristics in this case:
    \begin{itemize}
        \item Tile wrt L1 memory size 
        \item Tile wrt accelerator PE Array size
        \item Tile along certain dimensions of activations due to data layout in accelerator
    \end{itemize}
    \item Technique to reduce data copies to and from L1.
    \item Dory approach was adapted for coarse grained accelerator with minimal effort (writing template for coarse grained accelerator is relatively easy ;-) Ok @Alessio?)
          {\color{red} Should we also make claims about expandability of our approach here somewhere?}
    \item {\color{red}we should probably say something about the data layout of the accelerator ?}
\end{itemize}

==> text_bullets/Results.tex <==
\section{Experimental Results}
\input{tables/Table_Networks}
In this section we measure:
\begin{itemize}
    \item Cycle count using RISC-V cycle counters.
    \item Binary size using GNU \texttt{size}.
    \item Power consumption, measuring the average power consumption across different kernels.
    \item Compilation time ({\color{red}our compilation time is a lot faster than if we would need TVM to tune it, however it might be difficult to compare these})
\end{itemize}
{\color{red} Should we also report on runtime memory usage/ RAM?}

We do this each time for different scenarios:
\begin{itemize}
    \item Single layers:
        \begin{itemize}
            \item Conv2D
            \item Depthwise Separable Convolution
            \item Fully Connected layer
        \end{itemize}
    \item Full Networks of v0.7 of the MLperf\textsuperscript{TM} Tiny Benchmark suite:
    \begin{itemize}
        \item \texttt{DS-CNN} for Keyword spotting
        \item \texttt{MobileNet} for Visual Wake words
        \item \texttt{ResNet} for Image Classification
        \item \texttt{ToyAdmos} for anomaly detection
    \end{itemize}
\end{itemize}

{\color{red}
We can show these things:
\begin{itemize}
    \item Difference in cycles/binary/power when using different cores (Analog/Digital/RISC-V)
    \item Difference in cycles/binary/power when using different tiling strategies
    \item Difference in cycles/binary/power when turning on or off TVM optimizations
\end{itemize}
}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/Single_layers.png}
    \caption{Caption}
    \label{fig:my_label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{images/Ablation_tiling_cycles.png}
    \caption{Caption}
    \label{fig:my_label3}
\end{figure}
\subsection{Setup}
Figure \ref{fig:measurement_setup} shows the measurement setup.
\begin{figure}
    \centering
    \includegraphics[scale=0.05]{images/Experimental_setup.jpg}
    \caption{{\color{red}Maybe we need a better picture?} Placeholder for Measurement Setup}
    \label{fig:measurement_setup}
\end{figure}
\subsection{Cycles}
\subsubsection{Single Layer Deployment}
MAC/cycle vs operations on analog, digital, riscv core.\\
1. Show FC, DW, and Normal\\
2. show different scalability using more channels or bigger xy feature map\\
3. Show tiling advantages\\
4. add an ablation study on different accelerators? Simulating them
\subsubsection{TinyML Benchmarks}
performance on tinyML perf suit. We can run all the 4 networks also using the riscv core. We want to show for example that running DW on accelerator it does not make sense, but we should run on the risc-v core -- check MV1, check Fully-Connected (FC-AE).
\subsubsection{Compiler Optimizations}
1. optimization in network --> check when the layer can fit L1 and does not copy data to L2. Uneven mapping of layer after --> compare cycles\\
2. format optimization

\subsection{Binary size}
\subsection{Power consumption}


==> text_bullets/abstract.tex <==
%\begin{abstract}
%The efficient deployment of Deep Neural Networks (DNNs) on the extreme edge of the Internet-of-Things is critical to support deep-learning based applications.
%% 
%Modern AI-oriented edge-devices usually have limited on-chip memory, usually without a caching system.
%Furthermore, the computational hardware of these systems is typically composed of multiple heterogeneous compute cores to improve latency and energy efficiency, spanning from serial dispatching cores to highly parallel accelerators.
%Mapping modern DNNs on these systems is not trivial and requires a dedicated infrastructure to support the different components of the platform.
%%
%In this work, we propose \textit{HTVM} (\textit{...}) -- an automatic flow based on the open source TVM framework to deploy networks on AI-oriented edge platforms.
%%
%HTVM inherits the structure of TVM, ...
%As a case study for HTVM, we target Diana, a SoC caracterized by a two-level scratchpad memory and ..... 
%\end{abstract}


\begin{abstract}

Optimal deployment of Deep Neural Networks (DNNs) on heterogeneous compute platforms is a critical step in pushing the state-of-the-art for tiny machine-learning applications forward.

% ---- MVA: problem statement rephrased ----
% Modern SoCs for deep learning come with increasingly sofisticated compute capabilities of various kinds, including highly parallel MAC cores or even analog in-memory compute units. Efficiently mapping neural network operations onto the different compute modules in such heterogenous systems is therefore a challenging task. Additional considerations to optimally drive the whole system, like operator constraints, multi-level memory management and control over a large amount of intricate hardware details, makes this task extremely complex.

% 
State-of-the-art Systems-on-Chip (SoCs) for \mv{(extreme)} edge applications usually have limited and programmer-managed on-chip memory.
To further optimize for latency and energy efficiency, these SoCs can contain multiple heterogeneous compute cores, spanning from serial arithmetic cores to highly parallel accelerators.
%
The \mv{Wide variety in accelerator architectures and memory hierarchies, together with} the high amount %and depth 
of intricate details that need to be considered to optimally drive this hardware, %and achieve optimal performance 
make deployment a non-trivial task and performance assessment of different workloads impractical. 
%Mapping modern DNNs on these systems is not trivial and requires a dedicated infrastructure to support the different components of the platform.

% MVA ---- HTVM only works with diana, we should make this more clear here ----

In this work, we propose \textit{HTVM} %(\textit{...}) 
-- an %automatic optimized and 
extensible \mv{compilation} \mv{and optimization} flow to deploy DNNs on embedded SoCs \mv{consisting of a heterogeneous mix of microcontroller CPU cores and diverse accelerator cores. \textit{HTVM} is} based on the open source TVM\cite{chen2018tvm} and DORY\cite{burrello2021dory} frameworks, \mv{extended with parametrized pattern matchers to offload computational kernels to a heterogeneous set of accelerator at high utilization, and heuristics to minimize the memory and resource footprint}.
%\textit{HTVM} allows for quick deployment of different computational kernels on an embedded microcontroller CPU or offload to dedicated accelerator hardware,
%all while trying to keep the resource footprint as low, and hardware utilization as high possible.
Using \textit{HTVM}, we are able to deploy and measure the performance of various DNNs \mv{from the tinyMLperf benchmarking suite} on Diana\cite{ueyoshi2022diana}, an embedded SoC with a RISC-V CPU core, a digital AI \mv{accelerator as well as an} analog \mv{compute-in-memory AI} accelerator core with a two-level explicitly managed scratchpad memory. \mv{[Something quantitative?]}
%
%HTVM inherits the structure of TVM, ...
%As a case study for HTVM, we target Diana, a SoC caracterized by a two-level scratchpad memory and ..... 
    \end{abstract}

==> text_bullets/background.tex <==
\section{Background and Related Works}

{\color{red} This has to be scoped down by a lot, which other hardware/software is still relevant/important to compare to?}

Taxonomy of related works:

\textit{(Hardware choices are reflected in compilation strategies)}

\textbf{Hardware (XPUs, Accelerators, SoC's)}:
\begin{enumerate}
    \item Runtime resources
    \begin{itemize}
        \item Desktop/Cloud OS (Multiple VM support, Network support, lots of support for processes, dll's, ...)
        \item RTOS/Mobile OS (minimal processes)
        \item Bare-metal
    \end{itemize}
    \item Fine-grained vs coarse grained accelerator primitives/ dispatch possibilities (spectrum?)
    \begin{itemize}
        \item CPU PULP-NN \cite{garofalo2020pulp} and \cite{schiavone2018quentin}(SIMD ISA extensions)
        \item GPU (TensorCores?)
        \item Accelerator GEMM (TVM VTA \cite{moreau2019hardware}, GEMMini\cite{genc2021gemmini}, edgeTPU\cite{}, PULP-cluster\cite{})
        \item Accelerator Conv2D (Sirius, Diana)
    \end{itemize}
    \item Memory management
    \begin{itemize}
        \item Explicitly managed
        \item Hardware managed
    \end{itemize}
\end{enumerate}

(Mention FPGA implementations?)

\textbf{Software (Libraries, Compilers, Runtimes)}:
\begin{enumerate}
    \item Runtime resources:
    \begin{itemize}
        \item Lot's of resources: PyTorch\cite{paszke2019pytorch}, Tensorflow\cite{abadi2016tensorflow} or cloud: Horovod \cite{sergeev2018horovod}, PyTorch Lightning\cite{} \textit{(Runtime allocation/compilation)}
        \item Less resources: Tensorflow Lite \cite{}
        \item Even less resources: Tensorflow Lite Micro \cite{tflitemicro2021}, uTVM C runtime \cite{}, TinyIREE\cite{tinyiree2022} \textit{(ahead of time allocation/compilation, binary size critical)}
    \end{itemize}
    \item Fine-grained vs coarse grained accelerator primitives (Dispatch region selection)
    \begin{itemize}
        \item GCC/LLVM low level optimizations: LLVM IR
        \item Loop-level dispatch region selection: TVM TIR (CPU and GPU), {\color{red}TC-CIM\cite{siemienuk2021occ}\cite{vadivel2020tdo}\cite{drebes2020tc}
        \cite{lin2021accelerate}}
        \item Operation-level dispatch region selection: TVM BYOC\cite{chen2021bring}
        
        \item + Across different levels: MLIR-based\cite{} IR's, DaceML\cite{rausch2022data}, Interoperator Scheduling\cite{ding2021ios}
    \end{itemize}
    \item{Memory management}
    \begin{itemize}
        \item Explicitly optimized: Dory\cite{burrello2021dory}, Exo\cite{ikarashi2022exocompilation}, (TensorComprehensions\cite{vasilache2018tensor}? PolyHedral?)
            \item Implicitly optimized: TVM autotuner\cite{chen2018tvm}, TVM Ansor\cite{zheng2020ansor}
    \end{itemize}
\end{enumerate}

\textbf{Kernel Optimization methods Taxonomy}:
\begin{itemize}
    \item Manual optimization: NVIDIA CuDNN\cite{chetlur2014cudnn}, Intel OneDNN, ...
    \item Human-guided (DaCeML)
    \item Polyhedral optimization, TC-CIM, TensorComprehensions
    \item Feedback-directed/Profile-guided Optimization (PGO) (Online = Runtime Measurments):
    \begin{itemize}
        \item Memory layout aware: Exo (halidelike + Z3 SMT-solver for Equivalence proving)
        \item Memory layout unaware: Halide\cite{ragan2013halide}, TVM Autotuner (halidelike + coarse grained) = Treeboosting + scheduling templates, TVM Ansor = Genetic Algo (templateless). TVM Collage\cite{byungsoo2022collage}
    \end{itemize}
    \item Feedback-directed/Profile-guided Optimization (PGO) (Offline = Model measurements):
    \begin{itemize}
            \item Energy aware: Axonn ?(\cite{dagli2022axonn})
        \item Runtime/Cycle aware: MLIR/IREE SHARK (?) STONNE \cite{munoz2021stonne}(?)
    \end{itemize}
    \item Formalize as Linear Programming optimization + Heuristics: Dory (Memory-aware tiling)
    \item Neural Architecture Search (?) : MCUNet (Depth-first tiling) \cite{mcunet_2020}
\end{itemize}


%We choose
%
%Three main points (taxonomy):
%- explicitly vs cache memory;
%- fine-grained vs. corse grained;
%- design vs runtime scheduling

\textbf{Diana is a high-performance heterogeneous embedded SoC targetted towards edge NN inference with:}
\begin{enumerate}
    \item A low performance high-flexibilty, high-precision RISC-V CPU core
    \item A high-performance mid-precision Coarse-grained Digital CNN Accelerator
    \item An ultra-high performance low-precision Coarse-grained Analog In-memory Compute Accelerator
    \item 512 Kb L2 SRAM main on-chip memory
\end{enumerate}

\textbf{Diana demands {\color{red}(couple this back to what exists)}}:
\begin{itemize}
    \item Low memory usage, runtime overhead (both in size and cycles)
    \item Ahead-of-time compilation/parsing/allocation strategy (very few room for runtime compilation/ allocation overhead)
    \item Coarse grained dispatching (Fine grained does not make a lot of sense, except maybe for the CPU)
    \item Quantization aware model delivery (Future work, a lot of off the shelf compilers don't support s)
    \item Support for various backends (different accelerators with their own custom data layout)
    \item Explicit memory management. (Not all compilers support this)
    \item C code emission (due to practical constraints + to optimally use CPU ISA extension (Reuse GCC port, no XpulpV2 LLVM backend available))
\end{itemize}

%Focus on scarse resources, with coarse grained programming, explicit memory management to reduce runtime, and a lightweight runtime.
\textit{We introduce a new compiler that can deal with custom accelerators and memory management without hardware cache.}

%Some related work we should look into (by Josse):
%\begin{itemize}
%    \item Memory wall in MCU controllers
%    \begin{itemize}
%        \item Tiling - Dory: formulated as constraint optimization problem
%        \item Depth first tiling - MCUNET : Neural Architecture Search + TVM cascading compiler
%    \end{itemize}
%    \item Heterogeneous MCU - accelerator combinations
%    \begin{itemize}
%        \item Fine grained - TVM VTA + GEMMIni? + edgeTPU?(Systolic arrays and GEMM )
%        \item Coarse grained --> Diana/Sirius (Conv2D specific? ?
%    \end{itemize}
%    \item Infrastructure NN program transformation and execution
%        \item compilers:
%        \begin{itemize}
%            \item Halide-like --> TVM + Exo
%            \item polyhedral --> IREE??? (not really mentioned in paper how is optimized)
%            Some of the work of corporaal TC-CIM etc?
%        \end{itemize}
%        \item runtimes
%        \begin{itemize}
%            \item 
%        \end{itemize}
%\end{itemize}

%\begin{itemize}
%    \item https://github.com/mit-han-lab/mcunet (lots of papers!)
%    \item Arm cascading compiler https://github.com/apache/tvm-rfcs/blob/main/rfcs/0037-arm-ethosu-cascading-scheduler.md
%    \item diana paper: https://ieeexplore.ieee.org/document/9731716
%    \item dory paper: https://ieeexplore.ieee.org/document/9381618
%    \item TVM paper usenix
%    \item TVM VTA Accelerator https://tvm.apache.org/docs/topic/vta/index.html
%    \item Tensorflow Lite Micro related papers?
%    \item https://github.com/ucb-bar/gemmini and the exo-compiler https://dl.acm.org/doi/abs/10.1145/3519939.3523446
%    \item Edge tpu compiler https://coral.ai/docs/edgetpu/compiler/ (wehave one such board lying around)
%    \item TinyIREE bare metal deployment: https://arxiv.org/pdf/2205.14479.pdf
%    {\color{red}IREE puts a focus on binary size for their runtime and algorithms, should we do something similar? Report that we have a small binary size, regardless of }
%    \item Jetson Nano? https://blog.raccoons.be/coral-tpu-jetson-nano-performance
%    \item Vikram suggested DSAGEN (UCLA) and ESP (Columbia) and AHA (stanford)
%    \item TC-CIM related compilers https://research.google/pubs/pub48845/ and other H corporaal papers
%\end{itemize}

==> text_bullets/intro.tex <==
\section{Introduction}
%\cite{mcunet_2020}

\begin{itemize}
    \item There's a huge promise in AI inference performance on platforms like Diana\cite{ueyoshi2022diana} and TinyVers\cite{jain2022tinyvers}
    \item Diana deployment still daunting for end-users $\rightarrow$ limits application potential.
    \item Off-the-shelf toolchains/compilers insufficient
\end{itemize}

{\color{blue}

In our work, we propose the following contribution:


\begin{itemize}
    \item We show the limitations of current general-purpose or architecture-specific compilation chains. We demonstrate that an hybrid approach that exploits fraction of architecture-specific code on top of general-purpose one solve the problems of current tools, enlarging the space of supported networks, reducing the time-to-deploy for new networks, and achieving maximum performance.
    \item We propose and detail a new compilation flow based on the open source TVM to support heterogeneous compilation for neural networks, i.e., to dispatch neural networks layers to one or multiple accelerators comprised in the target architecture.
    \item We demonstrate the employment of our new compiler to deploy neural networks on Diana, a platform with a huge (max throughput xxx GMAC/s) and fast analog accelerator supporting ternary weights and a slower digital one (max throughput yyy GMAC/s).
\end{itemize}
}
{\color{red}Results here after.}
